Spatial Sharing of GPU for Autotuning DNN models

GPUs are used for training, inference, and tuning the machine learning models. However, Deep Neural Network (DNN) vary widely in their ability to exploit the full power of high-performance GPUs. Spatial sharing of GPU enables multiplexing several DNNs on the GPU and can improve GPU utilization, thus improving throughput and lowering latency. DNN models given just the right amount of GPU resources can still provide low inference latency, just as much as dedicating all of the GPU for their inference task. An approach to improve DNN inference is tuning of the DNN model. Autotuning frameworks find the optimal low-level implementation for a certain target device based on the trained machine learning model, thus reducing the DNN's inference latency and increasing inference throughput. We observe an interdependency between the tuned model and its inference latency. A DNN model tuned with specific GPU resources provides the best inference latency when inferred with close to the same amount of GPU resources. While a model tuned with the maximum amount of the GPU's resources has poorer inference latency once the GPU resources are limited for inference. On the other hand, a model tuned with an appropriate amount of GPU resources still achieves good inference latency across a wide range of GPU resource availability. We explore the causes that impact the tuning of a model at different amounts of GPU resources. We present many techniques to maximize resource utilization and improve tuning performance. We enable controlled spatial sharing of GPU to multiplex several tuning applications on the GPU. We scale the tuning server instances and shard the tuning model across multiple client instances for concurrent tuning of different operators of a model, achieving better GPU multiplexing. With our improvements, we decrease DNN autotuning time by up to 75 percent and increase throughput by a factor of 5.

==> my_packages.tex <==
%\setlength{\textfloatsep}{10pt plus 1.0pt minus 2.0pt}
%\setlength{\intextsep}{10pt plus 2pt minus 2pt}

%\usepackage{usenix,epsfig,endnotes}
%\usepackage{usenix,epsfig}
%\usepackage{booktabs}
%\usepackage{outlines}
%\usepackage{epsfig}
%\usepackage{graphicx}
%\usepackage[sort]{cite}  %resulting into errors with new ACM format.
%\usepackage[numbers,sort&compress]{natbib}
%\usepackage{cite}
%\usepackage{amsmath,amssymb,amsfonts}
%\usepackage{algorithmic}
%\usepackage{textcomp}
%\usepackage{xcolor}


%\PassOptionsToPackage{hyphens}{url}
%\usepackage[hyphens]{url}
%To keep the foot notes in the footer
%\usepackage[bottom]{footmisc}
%\usepackage{multirow}
%\usepackage[demo]{graphicx}
%\usepackage{caption}
%\usepackage{xspace} %\xspace
%\usepackage{lipsum}
%\usepackage{subcaption}
%\usepackage{amsfonts} % \checkmark
%\usepackage{subfig}
%\DeclareGraphicsExtensions{.png, .pdf, .jpg, .bmp}
%\usepackage{courier}

%\usepackage{filecontents}
%\usepackage{tikz}
%\usepackage{amsmath}

%\usepackage{graphicx}
%\usepackage{tabularx}
%\usepackage{multirow}
%\usepackage{balance}
%\usepackage{makecell}
%\usepackage{adjustbox}
%\usepackage{microtype}
 
%\usepackage{tcolorbox}
%\usepackage[font=small,skip=4pt]{caption}
%\usepackage[compact]{titlesec}
%\titlespacing*\section{0pt}{2.5ex}{1ex}
%\titlespacing*\subsection{0pt}{1.5ex}{0.5ex}
%\titlespacing*\subsubsection{0pt}{1ex}{0.5ex}

\usepackage{enumitem}
\setlist{topsep=1pt,itemsep=1pt,parsep=1pt,itemindent=0pt,leftmargin=0.13in}
\usepackage{outlines}

%Highlite capability
\usepackage{soul}
\soulregister\cite7
\soulregister\ref7

%For change Tracking
\usepackage{changes}


\newcommand{\mps}{CUDA MPS\xspace}
\newcommand{\cuda}{CUDA\xspace}
\newcommand{\nvidia}{NVIDIA\xspace}
\newcommand{\iml}{I\&ML\xspace}
\newcommand{\System}{DPDK based I\&ML node\xspace}
\newcommand{\manager}{I\&ML Manager\xspace}
\newcommand{\libml}{{\em libml}\xspace}
\newcommand{\mllib}{{\em libml}\xspace}
\newcommand{\ie}{{\em i.e., \/}}
\newcommand{\eg}{{\em e.g., \/}}
\newcommand{\etc}{{\em etc. \/}}
\newcommand{\etal}{{\em et al.\/}}

%\newcommand{\hide}[1] {}
\newcommand{\head}[1]{\vspace{1mm}\noindent{\bf #1}}
\renewcommand{\head}[1]{\vspace{1mm}\noindent{\it #1}}
% \renewcommand{\head}[1]{\vspace{1mm}\noindent{#1}}
\newcommand{\headbf}[1]{\vspace{1mm}\noindent{\bf #1}}
\newcommand{\netml}{Zero-Copy GPU scatter-gather\xspace}

\newcommand{\Scut}[1] {}
\newcommand{\Sshow}[1] {#1}
\newcommand{\mysec}[1]{\vspace{-2mm}\section{#1}\vspace{-2mm}}
\newcommand{\mysubsec}[1]{\vspace{-2mm}\subsection{#1}\vspace{-2mm}}
\newcommand{\myssubsec}[1]{\vspace{-2mm}\subsubsection{#1}\vspace{-2mm}}

\newcommand{\note}[1]{{\color{red}[#1]}}
\renewcommand\_{\textunderscore\allowbreak}
\newcommand{\mnote}[1]{{$\langle${\textcolor{red}{MA: \textbf{#1}}}$\rangle$}}
\newcommand{\twnote}[1]{{\color{red}[TW: #1]}}
\newcommand{\kknote}[1]{{\color{red}[KK: #1]}}
\newcommand{\knote}[1]{{\color{red}[KK: #1]}}
\newcommand{\pnote}[1]{{\color{red}[PS: #1]}}
\newcommand{\jwnote}[1]{{\color{red}[JC: #1]}}
\newcommand{\sknote}[1]{{\color{magenta}[SK: #1]}}
\newcommand{\anote}[1]{{\color{orange}[AD: #1]}}
\newcommand{\revisit}[1]{{\color{cyan}Check: #1}}
\newcommand{\findcite}[1]{\textcolor{magenta}{$^\text{[}$\footnote{\textcolor{red}{Find citation: #1}}$^\text{]}$}}
%\newcommand{\refine}[1]{\textcolor{blue}{[{\bf REFINE:} #1]}}
\newcommand{\newtext}[1]{{\color{red} \hl{NewText: #1}}}
%\newcommand{\trackchange}[1]{\textcolor{blue}{#1}}

\newcommand{\skfnote}[1]{\hide{{\color{magenta}[SK: #1]}}}
\renewcommand{\twnote}[1]{\hide{{\color{red}[TW: #1]}}}
%\renewcommand{\kknote}[1]{\hide{{\color{red}[KK: #1]}}}
%\renewcommand{\knote}[1]{\hide{{\color{red}[KK: #1]}}}
%\renewcommand{\srnote}[1]{\hide{{\color{red}[SR: #1]}}}
%\renewcommand{\jwnote}[1]{\hide{{\color{red}[JW: #1]}}}
%\renewcommand{\sknote}[1]{\hide{{\color{magenta}[SK: #1]}}}
%\renewcommand{\anote}[1]{\hide{{\color{orange}[AD: #1]}}}


\newcommand{\trackchange}[1]{\textcolor{blue}{#1}}
%\newcommand{\trackupdate}[1]{\textcolor{magenta}{{\bf} #1}}
\newcommand{\trackupdate}[1]{\textcolor{magenta}{#1}}
\newcommand{\trackupdates}[1]{\textcolor{green}{#1}}
\renewcommand{\trackchange}[1]{{#1}}
\renewcommand{\trackupdate}[1]{{#1}}
\renewcommand{\trackupdates}[1]{{#1}}

%Change the footnote to endnote.
%\renewcommand{\footnote}[1]{\endnote{#1}}

% Fix to reclaim the copyright space
%\makeatletter
%\def\@copyrightspace{\relax}
%\makeatother

\usepackage{booktabs} % For formal tables
\usepackage{listings}
\usepackage{color}
\usepackage{subcaption}
\usepackage{bytefield}
\usepackage[ruled, linesnumbered]{algorithm2e}
\SetKwComment{Comment}{$\triangleright$\ }{}
\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}

\lstset{frame=tb,
	language=C,
	aboveskip=3mm,
	belowskip=3mm,
	showstringspaces=false,
	columns=flexible,
	basicstyle={\small\ttfamily},
	numbers=none,
	numberstyle=\tiny\color{gray},
	keywordstyle=\color{blue},
	commentstyle=\color{dkgreen},
	stringstyle=\color{mauve},
	breaklines=true,
	breakatwhitespace=true,
	tabsize=3
}
%\usepackage{enumerate}
\hide{
Some Names and Acronyms:

}

==> sections/outline.tex <==
\jnote{Put notes if you have different thought or story of the paper.}
\Scut{
Key contributions in this paper.  
Finding the right resource allocation considering the inter-dependency between tuning procedure and inference for different models 
is important to maximize the powerful accelerator's utilization for both autotuning procedure and inference deployments
since the inter-dependency between autotuning procedure and inference during deployment in terms of different GPU resource allocation has not been explored. 
I think this paper is mainly about an analysis paper with some building system and enhancements based on findings.
So, we need to focus on results and explain them in details. 


I thinkn we need to highlight spatial sharing for autotuning (since paper title is also " Spatial Sharing of GPU for Autotuning DNN models) and then follow its correspoinding inference results with the context of autotuning.
The current version talks about inference with spatial sharing without context of autotuning. 
It makes me confuse the key parts and contents in the paper.

So, I would like to suggest the paper outline. 
They are not new and most of them are in the current version. 
We need to reorder and highlight them.


\begin{itemize}
    \item Show why we need sharing GPU resources for autotuning. 
    We can do more autotunings with one GPU at the same time and assign right resources for inference during deployment with the tuned model.
    \begin{itemize}
        \item Long autotuning time (e.g., Figure 1 (b) )
        \item Profile takes long time in overall autotuning procedures (cite TVM OSDI paper. That's why they developed ML part to avoid heavy cost of performing measurements)
        and requires several autotuning with different parameters (e.g., quantization) for the small model.
        \item Using multiple runner instances (i.e., using parallelism)) decreases total autotuning time. The way of increasing runner instances is using multiple physical GPUs or sharing one GPUs.
        However, using multiple physical GPUs without necessity may significantly increase costs due to its high cost plan (e.g., GPUs) in cloud enviromnet. 
        \item Sharing one GPU for autotuning is not explored yet since the accuracy of autotuning is the first priority to guarantee high performance inference.
    \end{itemize}
    \item We first explore various ways of sharing GPUs (e.g., temporal, spatial, and careful spatial sharing) with respect to autotuning procedures and analyze its impacts in details.
    Made a dicision that apatial sharing is a right way of autotuning due to secure (or accurate) autotuning results.
    \begin{itemize}
        \item Autotuning accuracy or inference results (e.,g, Fig 5)
        \item autotuning completion time
        \item resource utilization         
    \end{itemize}
    \item Expore inter-dependency between autotuning procedure and inference with spatial sharing and describe all observations. (Table1, 2,3 and Figure 2,3)
    \item Introduce a optimized system (e.g., long live server, monitoring systems) based on findings to enable things... Then, evalute the optimized system against others (e.g., Default TVM) (Fig 6 and Table 5)  
\end{itemize}
}

%we conduct an in-depth study of the impact the tuning of a model and latency at different amounts of GPU resources, revealing the underlying dependency.
%we explore the underlying causes that impact the tuning of a model at different amounts of GPU resources.
%We have observed an inter-dependency between the tuned model and its inference latency.
%A DNN model tuned with specific GPU resources provides the best inference latency when inferred with the same amount of GPU resources. However, a model tuned while having available the maximum amount of the GPU's resources has poorer inference latency once the GPU resources are constrained during inference. On the other hand, a model tuned with an appropriate amount of GPU resources still achieves good inference latency across a wide range of GPU resource availability during inference.
%Based on all these findings that share a GPU during tuning is helpful for increasing the throughput during tuning, we present techniques to spatially share a GPU such that a DNN model can be tuned at the desired percentage while also maximizing the utilization of the GPU resource.
\anote{Please see the following outline}
\jnote{Overall I think we have the same pages except for few things. I put my notes again.} 

Please see my outline. I think we should keep the emphasis on inference has to share GPU to use it more effectively and build up on that.
\knote{Whatever you folks do, please make sure that the paper has a good theme built around concrete, solid results to back up what we say. I appreciate the problem of having things that might be minor that we don't want to over-emphasize...}
\jnote{I did not mean that we do not emphasis on inference with sharing. I mean all contents or paper contribution are based on spatial sharing for autotuning and then its corresponding inferenece result and their inter-dependency. So, we have to be consistent for this theme and drive the story. Why do we want to talk about spatial inference sharing first without context of autotuing? I did not read this paper (Dynamic Space-Time Scheduling for GPU Inference)  carefully yet, but this paper discuss spatial sharing for inference and I thought there are many papers about them.. We need to put them as related works. Aditya: we have made the introduction give more importance to autotuning.}
I would rather like to shape the paper as:

1. Introduction: 
\begin{itemize}
\item Why is spatially sharing GPU necessary for both inference and tuning: can utilize GPU more efficiently, also can multiple tuning.
\knote{when? tuning? inference time? what is spatial inference? Don't you want to achieve best balance between inference latency and maximizing throughput during inference time?}
\item Why is tuning necessary. (Decreasing model inference latency)
\item What if we want to have both together, we could have GPU that is utilized well but also model that performs the best.
\item However, we have seen that we have to be cautious to use a tuned model as there is inter-dependency between how the model is tuned and how the model is inferred (on basis of GPU resources).
\end{itemize}

2. Background: 
\begin{itemize}
\item 1. More details on Autotuning, explain terms of TVM etc.
\item 2. More details on spatial sharing, explain how it runs on system, include CUDA MPS, environmental variable, limited number of SMs, compute isolation due to fixed GPU percentage.

\item \jnote{I think we first explain why we have to use spatial sharing for tuning here.. with existing experiment results by comparing temporal, default MPS and careful MPS. Then claim spatial sharing is a right way to go and focus on "spatial sharing impact on autotuning and inference. Aditya: I agree.}
\end{itemize}
3. Effect of Spatial Sharing on Tuning model
\begin{itemize}
    \item Table 2 and 3. Explain how the model tuned to certain percentage do get the best latency at that particular percentage. However, models tuned at 100\% has slower latency time at 25\% than model tuned at 50\%. Make a case that there is an appropriate GPU \% is a good point to tune a model.

\item Figure 2 and Figure 3: we go into details checking the amount of GPU resources (GPU threads each tuned model uses) and compare it with GFLOPS each model is tuned to. We have following observation:

\item Models get more efficient when tuned at less GPU\%. Model tuned with GPU\% of 25 achieves about 50\% GFLOPS of model tuned at 100\% GPU. - for the same result during inference? for about the same inference latency?

\item Model tuned at high GPU\% produce more threads. This is good when inferred at high GPU\% but when inferred at low GPU\%, the physical machine cannot run that many threads efficiently. However, the model tuned at lower percentage creates less threads which can be concurrently run better \knote{what does manage better mean?} in lower GPU\%, high number of threads can can cause timesharing in the SM. (We can compare to theoretical max GPU thread each \% of GPU can sustain).
\item Specific model wide focus. The heavier operating layers (Layers with * for mobilenet, and layers 1,3,6,9,12) for Resnet-18 show that GFLOPS of 50\% is quite close to model tuned at 100\% and GFLOPS of model tuned at 25\% is also about half of GFLOPS of model tuned at 100\%. Therefore, even a model tuned with small percentage can create quite a suitable model for inference.

\item Why do models tuned at 10\% do not produce the best model then? While the model might be most efficient (highest GFLOPS for thread), there are so few threads that when the model gets high amount of GPU, it cannot scale up to use all that GPU. 
\end{itemize}
\textbf{Conclusion of the section}: Lower percentage tuning can find a balance between GFLOPS and number of threads, therefore are suitable for inference with a wider range of GPU\%. However, with models such as VGG-19, which can effectively use all GPU compute resources due to compute heavy nature of the model, there is very little effect of tuning, thus, any percentage tuning is suitable. 
Show that inter-dependency of tuning and inference while spatial sharing exists in chameleon too. 
\knote{emphasize correctness of model irrespective of what \% it is tuned at. Aditya: Okay I will empasize that in relevent section.}

4. \textbf{How to Spatially share effectively?}
\begin{itemize}
    \item The performance gain in TVM comes with using more servers. More servers means more CPU side work done in parallel, thus, faster tuning time.

%\item We already recommend tuning model at lower GPU\%. Rest of the GPU is free. We could share that GPU with another TVM server to speed up tuning.

%\item But, share how? Temporal sharing and Default MPS can have interference so they pick wrong results. Figure (7).Rather we should have multiple servers but each server should have isolated section of GPU. \jnote{I am not sure, why do we bring temporal sharing here now. It is better to make claim that we need to use spatial sharing for tuning and then focus on all its impacts since all the contents for far are about spatial sharing..}

\item This the setup we want. (Explain with figure 6 (b)).

\item show that it can tune model faster than using just 1 server (obviously).

\item show you can rather split a single model in multiple sections (task 1-5 in one compute node, task 5-10 in another) and tune a model in 2 TVM servers spatially sharing GPU, we can effectively tune model much faster.
\end{itemize}
\knote{Are you bringing out a theme of the paper that says that you are also increasing throughput of the tuning process across one or more models being tuned concurrently with a certain amount of hardware, so that you can better use the cloud resources, if you are a cloud service provider offering tuning services on the expensive hardware? Aditya: yes, we will change the introduction appropriately to say such. }

\textbf{Conclusion of the Paper}: Explain that inference with spatial sharing not an explored territory for autotuning as well as the impact of tuning has on inference latency. 
. %\jnote{I am not clear what it means. Do you mean that spatial sharing for inference is not explored? Accurately, I think autoutuning with spatial sharing and its impact on inference (with also spatial sharing) are not explored..}
With model tuning being quite time consuming, tuning at certain good GPU\% once could result in a good functioning model, while also allowing us to do more work with GPU.

